GLIME: General, Stable and Local LIME Explanation

As black-box machine learning models grow in complexity and find applications in high-stakes scenarios, it is imperative to provide explanations for their predictions. Although Local Interpretable Model-agnostic Explanations (LIME) [22] is a widely adpoted method for understanding model behaviors, it is unstable with respect to random seeds [35,24,3] and exhibits low local fidelity (i.e., how well the explanation approximates the model's local behaviors) [21,16]. Our study shows that this instability problem stems from small sample weights, leading to the dominance of regularization and slow convergence. Additionally, LIME's sampling neighborhood is non-local and biased towards the reference, resulting in poor local fidelity and sensitivity to reference choice. To tackle these challenges, we introduce GLIME, an enhanced framework extending LIME and unifying several prior methods. Within the GLIME framework, we derive an equivalent formulation of LIME that achieves significantly faster convergence and improved stability. By employing a local and unbiased sampling distribution, GLIME generates explanations with higher local fidelity compared to LIME. GLIME explanations are independent of reference choice. Moreover, GLIME offers users the flexibility to choose a sampling distribution based on their specific scenarios.

==> main/gauss.tex <==
\section{GaussLIME: local and unbiased sampling distribution}
% \cref{sec:lime_unstable} illustrates that LIME is unstable because weights in LIME is close to zero when $\sigma$ is small and this makes regularization dominates the whole objective. By redefining LIME, we show theoretically that RedLIME, which is equivalent to LIME, converges much faster and is more stable.
In this section, we will show that LIME is actually biased in its sampling neighborhood and its explanation differs in terms of reference baseline $\*r$ which is chosen by users. Although RedLIME converges much faster than LIME, since they are equivalent in limit, RedLIME is also biased. We generalize the sampling neighborhood in LIME and present GaussLIME, which does not depends on $\*r$, by choosing an unbiased sampling distribution. 

\subsection{Sampling neighborhood in LIME is biased}\label[section]{sec:biased_lime}
\textbf{Biased sampling in LIME. }Recall in \cref{sec:original_lime}, LIME is essentially sampling from a hypercube determined by the instance $\*x$ to be explained and corresponding reference $\*r$. More specifically, to generate a neighborhood sample $x^\prime$ of $\*x$, LIME first sample $\*z$ uniformly from $\{0,1\}^d$, then $x^\prime_j = x_j, \forall j\in \{k:z_k =1\}$ and $x^\prime_j = r_j , \forall j \in \{k:z_k = 0\}$. Intuitively, only corner points on the hypercube could be sampled and these points all lie on the same side of $\*x$, i.e., the side where $\*r$ lies. Therefore, only the neighborhood on the same side with $\*r$ is considered which means sampling neighborhood is biased (see \autoref{fig:intro_full}). \emph{However, in order to characterize the local behavior of the model $f$, both the neighborhood on $\*r$'s side and that is not should be taken into account in sampling. } \cite{slack2020fooling} shows that LIME's perturbation distributes quite differently with the original data which could be leveraged to hide model bias. 

In addition, due to biased sampling, LIME returns different explanations with different references even for a linear model \cite{jain2022missingness, garreau2021does}. 
\begin{lemma}[Proposition 4 in \cite{garreau2021does}]
Suppose $\*x$ has $D$ pixels that is segmented into $d$ super-pixels $\{1,\cdots, d\}$, the reference vector is $\*r\in \mathbb{R}^D$. $f(\*x) = \sum_{k=1}^D c_k x_k$ is a linear model, then LIME explanation with infinitely many samples is $\*w^{\text{LIME}}_j = \sum_{k: k\in \text{ super-pixel }j} c_k (x_k - r_k), \forall j = 1,\cdots, d.$
\end{lemma}

Empirically, we illustrate LIME's dependence of reference in \cref{sec:diff_baseline}. It is clear that explanations with different reference rank super-pixels quite differently. 

% We choose six references: black image, white image, red image, yellow image, blue image and the average value of the super-pixel which is the default setting for LIME. For each image, we consider all pairs of these references and for each pair, we compute the jaccard index of their explanations and the average jaccard index across all pairs is reported. It is clear that explanations with different reference rank super-pixels quite differently. 

\textbf{Non-local sampling neighborhood.} As LIME aims to explain the local behavior of $f$, samples should be in the local neighborhood of $\*x$. Although in theory, LIME can generate samples close to $\*x$ and use $\pi(\cdot)$ to enforce locality, however, with limited budget, samples generated generally are distant from $\*x$ and thus locality cannot be enforced by weighting anyway. In \autoref{fig:sample_distance}, we plot the distribution of $\|\*x - \*x^\prime\|/\|\*x\|$ between sample $\*x^\prime$ and $\*x$ for different methods with sample size 1024. Samples generated by LIME is distant to $\*x$ which means $\*x^\prime$ is not in a local neighborhood of $\*x$. On the contrary, RedLIME and GaussLIME (introduced in the next section)  involve locality in sampling which enable them to generate local samples. Locality of them are controlled by $\sigma$. 
\begin{wrapfigure}{r}{5cm}
\centering 
\includegraphics[width=5cm]{imgs/sample_norm_dist_to_x.pdf}
         \caption{\textbf{Distribution of sample distance to original input. } $\*x$ is the original input and $\*x^\prime$ is a sample generated by different methods. LIME samples has a large distance with $\*x$ while RedLIME and GaussLIME samples are more local. When $\sigma$ is large no point close to $\*x$ is sampled by LIME and RedLIME. }
         \label{fig:sample_distance}
\end{wrapfigure}
\subsection{GaussLIME: unbiased local sampling}
LIME only samples corner points on the hypercube determined by reference $\*r$ and instance $\*x$. Therefore, as argued in \cref{sec:biased_lime}, a sampling neighborhood that is unbiased and enforce locality in a smoother way is required. 

Our solution to this is to choose a continuous distribution that is centered at $\*x$ in the interpretable space and points closer to $\*x$ have a larger probability to be sampled. Consider such a continuous distribution $\mathbb{Q}$, to draw a sample $\*x^\prime$ in the neighborhood of $\*x$, we first sample $\*z \sim \mathbb{Q}, \*z \in \mathbb{R}^d$, then $\*x^\prime= \*x + \*z$. Intuitively, $z_j$ represents the enhancement/weakening for super-pixels $s_j$ in $\*x$. To compute explanation on $\*x$, we draw $n$ samples $\{\*z_i\}_{i=1}^n \sim \mathbb{Q}$ and then find $\*w^{\text{GaussLIME}}_n$ that minimizes objective in \autoref{eq:red-lime}.

A natural distribution to choose is Gaussian distribution. By choosing $\mathbb{Q} = \mathcal{N}(\*1, \sigma^2 \*I)$, we introduce GaussLIME. All neighborhood points in the interpretable space are considered in GaussLIME while locality is enforced by $\sigma$. A small $\sigma$ means a smaller neighborhood is considered while a large $\sigma$ means a larger sampling neighborhood. $\sigma$ also serves as a trade-off factor between local explanation and global explanation. Explanation is more local when $\sigma$ is small while it is more global when $\sigma$ is large. The specific $\sigma$ to use should be determined by users.

In contrast with LIME, there is no reference involved in GaussLIME, and thus GaussLIME explanations are not affected by references. 
% Actually we have \cref{prop:gauss_lime}
% \begin{proposition}\label[proposition]{prop:gauss_lime}
% The explanation returned by GaussLIME for $f$ at $\*x$ with infinitely many samples is 
% \[
% \*w^{\text{GaussLIME}} = \frac{1}{\sigma^2}\mbe_{\*z\sim \mathcal{N}(\*1, \sigma^2 \*I)}[(\*z - \*1) f_{\*x}(\*z)].
% \]
% If $f(\*x) = \sum_{k=1}^D c_k x_k$ is a linear model w.r.t. pixels, we have $\*w^*_j = \sum_{k:k \in \text{ super-pixel }j} c_k x_k, \forall j=1,\cdots, d$.
% \end{proposition}

\subsection{Connection with Gradient and SmoothGrad}
Intuitively, \autoref{eq:red-lime} fit a linear model to approximate $f_{\*x}(\cdot)$ on the interpretable space. The sampling distribution $\mathcal{N}(\*1, \sigma^2 \*I)$ controls the neighborhood the linear model aims to fit. A large $\sigma$ fit a linear model that approximates $f_{\*x}(\cdot)$ in a large neighborhood while a small $\sigma$ fit a linear model that approximates $f_{\*x}(\cdot)$ in a small neighborhood. \emph{A natural question to ask is: If $\sigma \to 0$, does $\*w^{\text{GaussLIME}} \to \nabla_{\*z} f_{\*x}(\*z)|_{\*z=\*1}$?} Fortunately, this can be proved to be true. Furthermore, by Stein's lemma \cite{lin2019stein}, we can show that GaussLIME and SmoothGrad are equivalent with each other in the interpretable space. The intuition is that if we only want to approximate $f_{\*x}$ in a infinitesimals neighborhood of $\*x$, the slope of the optimal solution is $\nabla_{\*z} f_{\*x}(\*1)$. On the other hand, if we want to approximate $f_{\*x}$ in a large neighborhood, since $\nabla_{\*z} f_{\*x}(\*z)$ is optimal at $\*z$, the optimal solution in the neighborhood should be the weighted average of  $\nabla_{\*z} f_{\*x}(\*z)$ across $\*z$ in this neighborhood. 
\begin{proposition}\label[proposition]{prop:smooth-grad}
The explanation returned by GaussLIME for $f$ at $\*x$ with infinitely many samples is 
\[
\*w^{\text{GaussLIME}} = \frac{1}{\sigma^2}\mbe_{\*z\sim \mathcal{N}(\*1, \sigma^2 \*I)}[(\*z - \*1) f_{\*x}(\*z)] = \mathbb{E}_{\*z\sim \mathcal{N}(\*0, \sigma^2 \*I)}[\nabla_{\*z} f_{\*x}(\*1 + \*z)],
\]
which is SmoothGrad explanation at $\*1$ in the interpretable space. When $\sigma\to 0$, $\*w^{\text{GaussLIME}} \to \nabla_{\*z} f_{\*x}(\*z)|_{\*z = \*1}$.
\end{proposition}


==> main/stable_old.tex <==
\section{LIME can be stabilized by (re-)definition}\label[section]{sec:lime_unstable}
In this section, we show that the default implementation of LIME is unstable and may generate dramatically different explanations for different random seeds when $\sigma$ is small. We argue that it is because \emph{when $\sigma$ is small, weights for $\*z_i \neq \mathbf{1}$ are very small and the regularization term dominates the whole objective}. We provide theoretical justification to our argument. \textbf{By incorporating weighting into sampling, the redefined LIME (RedLIME) is stable even with only a few samples.} 

\subsection{RedLIME: redefine LIME by incorporating weighting into sampling}
Assume that we have enough samples to omit the influence of regularization term $\lambda \|\*w\|_2$ so that the original problem \autoref{eq:ori_lime} is equivalent to:
\begin{equation}\label{eq:eqivalence}
\begin{split}
   \mathop{\arg \max}_{\*v} &\frac{1}{n} \sum_{i=1}^n \pi(\*z_i) (f_{\*x}(\*z_i) - \*v^\top \*z_i)^2  \approx \mathop{\arg \max}_{\*v}\mathbb{E}_{\*z \sim \textbf{Uni}(\{0,1\}^d)}\bigg[\pi(\*z) (f_{\*x}(\*z) - \*v^\top \*z)^2\bigg] \\ 
    & = \mathop{\arg \max}_{\*v}\sum_{k=0}^d \mathbb{E}_{\*z\sim \textbf{Uni}(\{0,1\}^d)}\bigg[e^{\frac{k-d}{\sigma^2}} (f_{\*x}(\*z) - \*v^\top \*z)^2 \bigg| \|\*z\|_0 = k\bigg] \mathbb{P}(\|\*z\|_0 = k)\\
    & = \mathop{\arg \max}_{\*v}\sum_{k=0}^d \mathbb{E}_{\*z\sim \textbf{Uni}(\{0,1\}^d)}\bigg[(f_{\*x}(\*z) - \*v^\top \*z)^2 \bigg| \|\*z\|_0 = k\bigg] \frac{e^{\frac{k-d}{\sigma^2}}\mathbb{P}(\|\*z\|_0 = k)}{\sum_{l=0}^d e^{\frac{l-d}{\sigma^2}} \mathbb{P}(\|\*z\|_0 = l)}\\
    & = \mathop{\arg \max}_{\*v}\sum_{k=0}^d \mathbb{E}_{\*z\sim \textbf{Uni}(\{0,1\}^d)}\bigg[(f_{\*x}(\*z) - \*v^\top \*z)^2 \bigg| \|\*z\|_0 = k\bigg] \Tilde{\mathbb{P}}(\|\*z\|_0 = k)\\
    & = \mathop{\arg \max}_{\*v}\mathbb{E}_{\*z \sim \Tilde{\mathbb{P}}}\bigg[(f_{\*x}(\*z) - \*v^\top \*z)^2\bigg], \quad \Tilde{\mathbb{P}}(\*z, \|\*z\|_0 = k) = \frac{e^{\frac{k}{\sigma^2}}}{(1 + e^\frac{1}{\sigma^2})^d} \\ 
\end{split} 
\end{equation}
We use $\Tilde{\mbp}$ to define RedLIME as follows: to generate a sample $\*z_i$, we first sample $k\in\{0, \cdots, d\}$ with probability $e^{\frac{k}{\sigma^2}}/(1 + e^\frac{1}{\sigma^2})^d$ and then sample $\*z_i$ uniformly from $\{\*z|\|\*z\|_0 = k\}$ and finally:
\begin{equation}\label[equation]{eq:red-lime}
   \*w^{\text{RedLIME}}_n = \mathop{\arg \min}_{\*v} \sum_{i=1}^n (f_{\*x}(\*z_i) - \*v^\top \*z_i)^2 + \lambda \|\*v\|_2^2 = (\sum_{i=1}^n \*z_i\*z_i^\top + \lambda \*I)^{-1} \big(\sum_{i=1}^n \*z_i f_{\*x}(\*z_i)\big).
\end{equation}
It is easy to see that when $n\to\infty$, LIME and RedLIME return the same solution $\*w$. We can derive the exact expression for this limit and show that when regularization is not present, LIME and RedLIME converge to $\*w$ at the same rate.
% By a similar derivation as \citet{garreau2021does}, we have the exact expression of $\*w$ in the following \cref{prop:exact:redlime}:
\begin{proposition}\label[proposition]{prop:exact:redlime}
When sample size $n\to\infty$, the explanation ${\*w}_n^{\text{LIME}}, {\*w}_n^{\text{RedLIME}}\to  \mbe_{\*z\sim \Tilde{\mbp}}[( \beta_2\*z + \beta_1 \*1)f_{\*x}(\*z)]$ where $\beta_1 = -1 - e^{\frac{1}{\sigma^2}}, \beta_2 = (1+e^{\frac{1}{\sigma^2}})^2/e^{\frac{1}{\sigma^2}}$. 

If $\lambda = 0$, $\forall \epsilon > 0, \delta \in (0,1)$, when $n = \Omega(\epsilon^{-2}d^2(1+e^{-\frac{1}{\sigma^2}})^2 \log(8d/\delta))$, we have $\mbp(\|\*w_n^{\text{LIME}} -\*w^{\text{LIME}} \| \geq \epsilon) \leq  \delta $ and $\mbp(\|\*w_n^{\text{RedLIME}} -\*w^{\text{RedLIME}} \| \geq \epsilon) \leq \delta $.
\end{proposition}
However, as presented in \autoref{fig:intro_example} and \autoref{fig:ji_full}, LIME is unstable and converges much slower than RedLIME especially when $\sigma$ is small. We show in the the next section that this is due to the interplay between weighting and regularization in LIME.

\subsection{LIME is unstable because weights are too small}
As discussed by previous works \cite{zafar2019dlime, shankaranarayana2019alime, visani2022statistical, zhou2021s}, LIME is unstable to random seeds. We show theoretically that this is because weights are too small and regularization dominates. As a consequence, explanation is close to zero. RedLIME requires much less samples to escape from the regime where regularization dominates and thus converges much faster. We will show empirical results on the effect of regularization and weighting in \cref{sec:experiments}.

% \subsubsection{Empirical findings}
% \textbf{Setup.} We sample 100 images from ImageNet and compute explanations for these samples on ResNet18 and small Swin-Transformer. To measure the stability of explanation methods, for each method and each sample, we compute explanations under 10 random seeds and compute the Jaccard Index for top-$k$ features for each pair of explanations and finally report the average Jaccard Index across $k=1,\cdots, d$ for each sample.

% \textbf{LIME is inconsistent while RedLIME is consistent.} \autoref{fig:intro_example} shows explanations computed on an example image under two different random seeds. $2^{14}$ samples are sampled and $\sigma=0.25$. The average jaccard index is shown for each method. Clearly, LIME shows inconsistent explanations while RedLIME presents much more consistent explanations.
\begin{wrapfigure}{r}{5cm}
\centering 
\includegraphics[width=5cm]{imgs/sample_norm_dist.pdf}
\caption{\textbf{Probability distribution and weight of $\|\*z_i\|_0$.} $\|\*z_i\|_0$ of samples generated by LIME follows binnomial distribution which is independent of $\sigma$. When $\sigma$ is small, distribution of $\|\*z_i\|_0$ generated by RedLIME concentrates at $d$ while samples in LIME all have non-negligible weight except those equal to $\*1$. When $\sigma$ is large, distribution of $\|\*z_i\|_0$ generated by RedLIME tends to binomial distribution while samples in LIME all have non-negligible weight.}
\label{fig:sample_norm_dist}
\end{wrapfigure}
\textbf{Sample weights are too small for LIME. }We plot the distribution of the ratio of non-zero elements to the number of super-pixels of samples and the corresponding weight for LIME and RedLIME in \autoref{fig:sample_norm_dist}. Clearly, most samples have $\approx \frac{d}{2}$ non-zero elements. However, when $\sigma=0.25$ or 0.5, almost all samples have weight close to zero. For example, when $\sigma=0.25$, then for $\|\*z\|_0 = \frac{d}{2}$, $\pi(\*z) = \exp(-8d)$ which is approximately $10^{-139}$ when $d=40$. Even if $\|\*z\|_0 = d-1, \pi(\*z) = e^{-16}\approx 10^{-7}$. Since regularization strength $\lambda=1$ by default, this implies that when we only have $<10^7$ samples, the first term in \autoref{eq:ori_lime} is dominated by the regularization term which leads to $\|\*w\|\approx 0$. 

\textbf{LIME needs exponentially more samples than RedLIME to omit the influence of regularization.} By explicitly incorporating weighting into sampling, all samples have weight 1. Thus, all samples are effective in \autoref{eq:red-lime}. And this cause RedLIME to require much less samples than LIME to escape the regime where regularization dominates. 
% \textbf{RedLIME is much more stable than LIME when $\sigma$ is small.} \autoref{fig:intro_full} presents Jaccard Index under different sample size $n$ and kernel width $\sigma$. When $\sigma=0.25$ which is the default value, with $2^{14}$ samples, the jaccard index of LIME is about 0.4 while that of RedLIME is close to 1 which means RedLIME ranks different features almost the same regardless of random seeds. RedLIME achieves jaccard index of over 0.55 even with only 32 samples. By examining the weight function $\pi(\cdot)$, we find that when $\sigma$ is small, almost all samples have weight close to zero. Since by default, the regularization parameter $\lambda$ is set to 1, the regularization term dominates the sum-of-square term in LIME. For example, when $\sigma=0.25$, since a sample $\*z_i$ generated by LIME is most likely to have $\|\*z_i\|_0 = \frac{d}{2}$ as shown in \autoref{fig:sample_norm_dist}, then $\pi(\*z_i) = \exp(-8d)$ which is approximately $10^{-139}$ when $d=40$. Even if $\|\*z_i\|_0 = d-1, \pi(\*z_i) = e^{-16}\approx 10^{-7}$. This implies that when we only have $<10^7$ samples, the first term in \autoref{eq:ori_lime} is dominated by the regularization term which leads to $\|\*w\|\approx 0$. In addition, \textcolor{blue}{concentration of $\hat{\*w}$ is much slower and thus LIME is unstable when only limited samples are available.}

% \textbf{RedLIME is equivalent to LIME for large $\sigma$ and large sample size $n$.} RedLIME outperforms LIME for different $\sigma$ but the stability improvement decreases when $\sigma$ becomes larger and more samples are generated. Actually, we will show that they are actually equivalent when we have infinite samples. Empirically, we also find that explanations computed by \textcolor{blue}{ LIME and RedLIME converges to the same value (see)}. As presented in \autoref{fig:sample_norm_dist}, when $\sigma$ is large, distributions of $\|\*z_i\|_0$ in LIME and RedLIME are close to each other. In this regime, $\pi(\*z_i)$ is of order $10^{-1}\sim 1$. For example, when $\sigma=5, d=40, \|z_i\|_0 = 0$, $\pi(\*z_i) \approx 0.2$. Hence, the first term in \autoref{eq:ori_lime} dominates the second term. In this case, we may omit the second term and find that \textcolor{blue}{$\*w_n$ concentrate faster.}

% \subsubsection{Theoretical justification}
% It has been shown that when regularization term is omitted, LIME and RedLIME have the same convergence rate. However, how many samples are needed to omit regularization? We will prove that LIME needs exponentially more samples than RedLIME to omit the impact of regularization and thus LIME converges exponentially slower when regularization is present which is stated in \cref{thm:over_regularization}.
\begin{theorem}\label[theorem]{thm:over_regularization}
    Suppose in LIME we have samples $\{\*z_i\}_{i=1}^n \sim \text{Uni}(\{0,1\}^d)$. For any $t >0, \delta \in (0,1)$, if $n = O\bigg(\lambda t \bigg(\frac{2e^{\frac{1}{\sigma^2}}}{1+e^{\frac{1}{\sigma^2}}}\bigg)^{d-1}\sqrt{\log\frac{1}{\delta}}\bigg),$    we have $\mbp(\sum_{i=1}^n \pi(\*z_i)\|\*z_i\|_0< t{\lambda}) \geq 1 - \delta $.
    
    Suppose in RedLIME we have samples $\{\*z_i\}_{i=1}^n \sim \Tilde{\mbp}$. For any $t >0, \delta \in (0,1)$, if $n = O\bigg(\lambda t \sqrt{\log\frac{1}{\delta}}\bigg),$ we have $\mbp(\sum_i\|\bz_i\|_0/d  < t{\lambda }) \geq  1-\delta.$
\end{theorem}

In \cref{thm:over_regularization}, $\sum_{i=1}^n \pi(\*z_i)\|\*z_i\|_0/d$ can be regarded as the coefficient of $\|\*v\|^2$ in the sum-of-square term in \autoref{eq:ori_lime} where $\lambda$ is the regularization coefficient of $\|\*v\|^2$. Hence, \cref{thm:over_regularization} demonstrates that LIME needs $O\big(\lambda t ({2e^{\frac{1}{\sigma^2}}}/{(1+e^{\frac{1}{\sigma^2}}}))^{d-1}\sqrt{\log\frac{1}{\delta}}\big)$ samples for the first term to be comparable with the regularization strength. However, on the other hand, RedLIME only needs $O\big(\lambda t \sqrt{\log\frac{1}{\delta}}\big)$ samples to achieve the same. LIME requires exponentially more samples than RedLIME which may cause LIME converges exponentially slower especially when $\sigma$ is small and $d$ is large as $({2e^{\frac{1}{\sigma^2}}}/{(1+e^{\frac{1}{\sigma^2}}}))^{d-1}$ is close to $2^{d-1}$ when $\sigma$ is small. 

\textbf{Explanation is close to zero when regularization dominates.} When regularization dominates, in order to minimize \autoref{eq:ori_lime} or \autoref{eq:red-lime}, explanations should be close to zero which may leads to less meaningful and unstable explanations. The following theorem proves that LIME requires exponentially more samples than RedLIME to return meaningful explanations. 
\begin{theorem}\label[theorem]{thm:close_to_zero}
For any $\epsilon , \delta \in (0,1)$, when sample size used in LIME satisfies
\[
n = O\bigg(\lambda \epsilon d^{-0.5}\bigg(\frac{2e^{\frac{1}{\sigma^2}}}{1+e^{\frac{1}{\sigma^2}}}\bigg)^d\sqrt{\log\frac{1}{\delta}}\bigg),
\]
we have LIME explanation is close to zero with high probability, i.e., $\mathbb{P}(\|\bw^{\text{LIME}}_n\|_2 < \epsilon) \geq 1- \delta$.

When sample size used in RedLIME satisfies
\[
n = O\bigg(\lambda \epsilon d^{-1}\sqrt{\log\frac{1}{\delta}}\bigg),
\]
we have RedLIME explanation is close to zero with high probability, i.e., $\mathbb{P}(\|\bw^{\text{RedLIME}}_n\|_2 < \epsilon) \geq 1- \delta$.
\end{theorem}

\cref{thm:close_to_zero} shows that when we only have a few samples, the explanation is close to zero. The sample complexity bound of LIME depends on $({2e^{\frac{1}{\sigma^2}}}/({1+e^{\frac{1}{\sigma^2}}}))^d$ which grows exponentially w.r.t $d$ and when $\sigma$ is small, it grows approximately in order $2^d$. Hence, this implies that when $\sigma$ is small, LIME explanation is close to zero even we have a lot of data. With the same sample size, RedLIME returns more meaningful explanation than LIME. 

\begin{remark}
Our discussion above suggests that using weighting to enforce locality may not be good when regularization is present. However, this does not means regularization is not necessary. When we only have $n < d$ data, regularization is actually beneficial for otherwise the problem is low-rank and ill-conditioned. More discussion on the effect of regularization in LIME can be found in .
\end{remark}


